Convolutional Filtering and Neural Networks with Non Commutative Algebras

In this paper we introduce and study the algebraic generalization of non commutative convolutional neural networks. We leverage the theory of algebraic signal processing to model convolutional non commutative architectures, and we derive concrete stability bounds that extend those obtained in the literature for commutative convolutional neural networks. We show that non commutative convolutional architectures can be stable to deformations on the space of operators. We develop the spectral representation of non commutative signal models to show that non commutative filters process Fourier components independently of each other. In particular we prove that although the spectral decompositions of signals in non commutative models are associated to eigenspaces of dimension larger than one, there exists a trade-off between stability and selectivity, which is controlled by matrix polynomial functions in spaces of matrices of low dimension. This tradeoff shows how when the filters in the algebra are restricted to be stable, there is a loss in discriminability that is compensated in the network by the pointwise nonlinearities. The results derived in this paper have direct applications and implications in non commutative convolutional architectures such as group neural networks, multigraph neural networks, and quaternion neural networks, for which we provide a set of numerical experiments showing their behavior when perturbations are present.

==> figures/50_asp_FilterClasses.tex <==
%!TEX root = ../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}




%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}


%-- Fifth color palette
\definecolor{my_cp5_col1}{RGB}{7, 117, 232}
\definecolor{my_cp5_col2}{RGB}{144, 171, 229}
\definecolor{my_cp5_col3}{RGB}{30, 73, 164}
\definecolor{my_cp5_col4}{RGB}{158, 158, 100}
\definecolor{my_cp5_col5}{RGB}{193, 195, 199}
\definecolor{my_cp5_col6}{RGB}{83, 83, 83}






\usetikzlibrary{positioning,decorations.pathreplacing,shapes}
%\usepackage[english]{babel}
%\usepackage{microtype}
%\usepackage[hmargin=1.5cm,vmargin=1cm]{geometry}
%\usepackage{amsmath}
%\DeclareMathOperator{\p}{p}
%\newcommand*{\cancer}{\text{cancer}}
%\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {1.3}
\def \unit  { \scale cm}
\def \layerinterdist {2.5}


% Block styles
\tikzstyle{set} = [rectangle,color=black,
                    rounded corners = 0.2*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]

                    
\tikzstyle{vectorspace} = [ set, 
                             fill=my_alejocol4c!50,
                             minimum width  = 1.5*\unit,
                             minimum height = 2.0*\unit]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=black!15,
                              minimum height = 1.3*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol2b!50,
                        minimum width = 1.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.05*\unit,
                    fill=black,
                    color=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]





{\fontsize{8}{8}\selectfont


\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% First state of processing%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Vector space M
   %\path (0,0) node [vectorspace, fill=my_cp4_col4] (M0) {};
   %\path (M0.south) ++ (0, 0) node [above, color=black] {$\mathcal{M}$};
   \path (0,0) node [] (M0) {};
   
   % Element of the vector space
   %\path (M0) ++ (-0.5,0.2) node [dot] (x) {};
   %\path (x.south)++(0,-0.1) node [below, color=black] {$\mathbf{x}$}; 
   
   % Element filtered in the vector space
   %\path (M0) ++ (0.5,0.2) node [dot] (ex) {};
   %\path (ex.south) node [below, color=black] {$\rho(a)\mathbf{x}$};      
              

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Space of endomorphisms
   \path (M0.north) ++ (0, 0.5) 
         node [endomorphisms, anchor=south, fill=my_cp4_col3] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below, color=black] {$\text{End}(\mathcal{M})$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3) node [dot] (e) {};      
   %\path (e) node [below] {$\rho_{0}(g)=\mathbf{S}_{0}$};    
   
%   % Arrow going from x to Ex
%   \path (e)+(-0.5,0.55) coordinate (c1);
%   \path (e)+(0.5,0.55) coordinate (c2);   
%   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   % Algebra_tilde
   \path (End0.north west) ++ (-3.5, 0) 
         node [algebra, anchor = north east, fill=my_cp4_col3] (At) {};   
   \path (At.north) ++ (0,-0.1) node [below,color=black] {$\tilde{\mathcal{A}}$};  
   
   % Subset in A_tilde  
    \path (At.south) ++ (0,0.1) 
    node [subendomor2in1, anchor=south,color=gray!20] (subset2) {};
    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\tilde{\mathcal{C}}$};
    
    % Element in the Algebra
    \path (subset2.south) ++ (0.0, 0.2) node [dot] (a2) {}; 
   
   % Algebra A
   \path (End0.north west) ++ (-1, 0) 
         node [algebra, anchor = north east, fill=my_cp4_col1] (A) {};   
   \path (A.north) ++ (0,-0.2) node [below,color=black] {$\mathcal{A}$};  
    
    % Subset in the Algebra  
    \path (A.south) ++ (0,0.1) 
    node [subendomor2in1, anchor=south,color=gray!20] (subset2) {};
    \path (subset2.south) ++ (0, 0.2) node [above, color=black] {$\mathcal{C}$};
    
    % Element in the Algebra
    \path (subset2.south) ++ (0.0, 0.2) node [dot] (a1) {}; 
        
   % Arrow indicating \rho going from A to End(M)  
   \path (A.north) + (0.5,-0.5) coordinate (c1);
   \path (End0.north) + (-0.5,-0.5) coordinate (c2);   
   \path [draw, -stealth,line width = 1.0,color=my_cp4_col2] (a1) .. controls (c1) and (c2) .. (e) node[midway,above left,rotate=0,color=my_cp4_col2] {$\rho$};
   
   % Arrow going from subset of A_tilde to subset of A
   \path (A.south) + (-0.2,-0.5) coordinate (c2);
   \path (At.south) + (0.2,-0.5) coordinate (c1);   
   \path [->,draw, -stealth,line width = 1.0,color=gray] (a2) .. controls (c1) and (c2) .. (a1) node[midway,below,rotate=0,color=gray] {$\iota$};




\end{tikzpicture}


}







==> figures/cqn.tex <==
% !TEX root = ../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}


%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}


%-- Fifth color palette
\definecolor{my_cp5_col1}{RGB}{7, 117, 232}
\definecolor{my_cp5_col2}{RGB}{144, 171, 229}
\definecolor{my_cp5_col3}{RGB}{30, 73, 164}
\definecolor{my_cp5_col4}{RGB}{158, 158, 100}
\definecolor{my_cp5_col5}{RGB}{193, 195, 199}
\definecolor{my_cp5_col6}{RGB}{83, 83, 83}


\def \myfactor {0.65}
\def \unit  {\myfactor cm}

% Definition of a block for block diagrams
\tikzstyle{block} = [ rectangle,
                      minimum width = \unit,
                      minimum height = \unit,
                      fill = gray,
                      draw = black,
                      text = black]

% Control the color and size of filter blocks                  
\tikzstyle{filter} = [block,
                      minimum width  = 3.0*\unit,
                      minimum height = 1.3*\unit,
                      fill=my_cp4_col1]

% Control the color and size of nonlinearity blocks 
\tikzstyle{nonlinearity} = [ filter,
                             minimum width  = 3.0*\unit,
                             fill = my_cp4_col3]

% Control the color and size of nonlinearity blocks 
\tikzstyle{pooling} = [ filter,
                             minimum width  = 3.0*\unit,
                             fill = my_cp4_col4]



% Control separation between blocks
\def \deltainput     {( 0.0,-1.7)}
\def \deltaoutput    {( 0.0,-1.2)}
\def \deltalayer     {3}
\def \deltaconnector {1}
\def \deltasigma     {( 4.5, 0.0)}

% The text that is displayed inside of filter blocks
\def \one   {$\displaystyle{\mathbf{h}_{1}  = \sigma\left(\mathbf{\hat{W}}_1 \ast \mathbf{h}\right)}$}
\def \two   {$\displaystyle{\mathbf{h}_{2}  = \sigma\left(\mathbf{W}_2 \ast \mathbf{h}_1\right)}$}
\def \three {$\displaystyle{\mathbf{h}_{3}  = \sigma\left(\mathbf{W}_3 \ast \mathbf{h}_2\right)}$}
% The text that is displayed inside of nonlinearity blocks
\def \sigmaone   {\normalsize{Quat Dense}}
\def \sigmatwo   {\normalsize{Quat Dense}}
\def \proyone   {\normalsize{Quat Dense}}
\def \proytwo   {\normalsize{Readout}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN FIGURE CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
{\fontsize{7}{7}\selectfont\begin{tikzpicture}[scale = \myfactor]

  \pgfdeclarelayer{bg}     % declare background layer
  \pgfsetlayers{bg,main}   % set the order of the layers (main is the standard layer)

  % Draw input to GNN
  \node (input) [rectangle, minimum width = 0.1*\unit] {$\mathbf{h}$};
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 1 Filter block and Feature block
  \path (input.east)      ++ \deltainput node [filter]       (L1 Filter1) {\one};
  \path (L1 Filter1) ++ \deltasigma node [filter] (L1 F1)      {\two};
  \path (L1 F1) ++ \deltasigma node [filter] (L1 F2)      {\textcolor{black}{\three}};
  % Draw connectors for Layer 1
  %\path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{z}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 Filter1.east) -- node [above] {$\mathbf{h}_1$} (L1 F1.west);
  \path[draw, -stealth] (L1 F1.east) -- node [above] {$\mathbf{h}_2$} (L1 F2.west);


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Layer 2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Draw Layer 2 Filter block and Feature block
  \path (L1 Filter1) ++ (0,-\deltalayer) node [nonlinearity]       (L2 Filter1) {\sigmaone};
  \path (L2 Filter1) ++ \deltasigma      node [nonlinearity] (L2 F1)      {\sigmatwo};
  \path (L2 F1) ++ \deltasigma node [pooling] (L2 F2)      {\textcolor{black}{\proytwo}};
  % Draw connectors for Layer 2
  \path[draw, -stealth] (L2 Filter1.east) --  node [above] {$\mathbf{y}_1$} (L2 F1.west);
  \path[draw, -stealth] (L2 F1.east) -- node [above] {$\mathbf{y}_2$} (L2 F2.west);  
  


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Connections across layers %%%%%%%%%%%%%%%%%%%%%%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % From input to layer 1
  \path[draw, -stealth] (input.east) -- (L1 Filter1.north);
  % From layer 1 to layer 2
  \path (L1 F2.south) ++ (0,-\deltaconnector) node [] (aux1) {};
  \path[draw, -stealth] (L1 F2.south) -- node [below right] {$\mathbf{h}_3$} (aux1.north) 
                                      --                         (aux1.north -| L2 Filter1.north) 
                                      -- node [above left]  {$\mathbf{h}_3$} (L2 Filter1.north);
  % From layer 3 to output
  \path[draw, -stealth] (L2 F2.south) -- ++ \deltaoutput -- ++ (0.5, 0) 
                        node [right]{$\mathbf{z}$};




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Light shades to signify layer groups   %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{pgfonlayer}{bg} 
% Shading for Layer 1  
\path (L1 Filter1.west |- L1 F1.south) ++ (-0.4,-0.35)
node [filter, anchor = south west,
fill = black!5, 
%minimum width  = 10.75*\unit,
minimum width  = 13*\unit,
minimum height = 2*\unit,] 
(layer)
{}; 
\path (layer.south west) ++ (0.0,0.0) node [above right] {};
% Shading for Layer 2  
\path (L1 Filter1.west |- L2 F1.south) ++ (-0.4,-0.35)
node [filter, anchor = south west,
fill = black!5, 
%minimum width  = 10.75*\unit,
minimum width  = 13*\unit,
minimum height = 2*\unit,] 
(layer)
{}; 
\path (layer.south west) ++ (0.0,0.0) node [above right] {};
 
\end{pgfonlayer}








\end{tikzpicture}} 


==> figures/fig13_embedded.tex <==
% !TEX root = ../compiler_paper.tex



%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Blue Colors of the Palette
\definecolor{my_alejocol5a}{RGB}{1,31,75}
\definecolor{my_alejocol4a}{RGB}{3,57,108}
\definecolor{my_alejocol3a}{RGB}{0,91,150}
\definecolor{my_alejocol2a}{RGB}{100,151,177}
\definecolor{my_alejocol1a}{RGB}{179,205,224}

%--------Red Colors of the Palette
\definecolor{my_alejocol4b}{RGB}{212, 220, 220}
\definecolor{my_alejocol3b}{RGB}{113, 18, 55}
\definecolor{my_alejocol2b}{RGB}{236, 85, 141}
\definecolor{my_alejocol1b}{RGB}{225, 73, 132}

%--------Blue-Green Colors of the Palette
\definecolor{my_alejocol4c}{RGB}{81, 185, 239}
\definecolor{my_alejocol3c}{RGB}{119, 164, 211}
\definecolor{my_alejocol2c}{RGB}{193, 223, 213}
\definecolor{my_alejocol1c}{RGB}{53, 89, 85}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}

%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

%-- Fifth color palette
\definecolor{my_cp5_col1}{RGB}{7, 117, 232}
\definecolor{my_cp5_col2}{RGB}{144, 171, 229}
\definecolor{my_cp5_col3}{RGB}{30, 73, 164}
\definecolor{my_cp5_col4}{RGB}{158, 158, 100}
\definecolor{my_cp5_col5}{RGB}{193, 195, 199}
\definecolor{my_cp5_col6}{RGB}{83, 83, 83}










\usetikzlibrary{positioning,decorations.pathreplacing,shapes}


\newcommand*{\cancer}{\text{cancer}}
\newcommand*{\testp}{\text{test}+}



%%%%%%%%%%%%%%%%%%%%%%%%%%% Settings of Blocks and picture %%%%%%%%%%%%%%%%%%%

\def \scale {0.75}
\def \unit  { \scale cm}
\def \layerinterdist {4.2*\unit}


% Block styles
\tikzstyle{set} = [rectangle,
                    rounded corners = 0.2*\unit,
                    fill=black!15,
                    inner sep=0pt,
                    draw,
                    anchor = center,
                    line width=0.1mm]

                    
\tikzstyle{vectorspace} = [ set,
                             minimum width  = 3.5*\unit,
                             minimum height = 2.5*\unit,
                             fill=my_cp4_col4 ]
                             
\tikzstyle{endomorphisms} = [ vectorspace,
                              fill=my_cp4_col3,
                              minimum height = 2*\unit]
                                
%%---subsets of Endomorphisms                               
\tikzstyle{subendomor2in1} = [endomorphisms, rounded corners=0.3*\unit,
                              fill=black!30,
                              minimum width  = 0.8*\unit,
                              minimum height = 0.8*\unit
                             ]                                                                                                                                                
\tikzstyle{algebra} = [ endomorphisms,
                        fill=my_alejocol1c,
                        minimum width = 1.5*\unit]


\tikzstyle{dot} = [ circle,
                    minimum width  = 0.1*\unit,
                    fill=black,
                    inner sep=0pt,
                    draw,
                    anchor = center ]






{\fontsize{8}{8}\selectfont

\begin{tikzpicture}[rounded corners,ultra thick]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% FIRST COLUMN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

   % Vector space EndM
   \path (0,0) node [vectorspace] (M0) {};
   \path (M0.south) ++ (0, 0) node [above] {$\text{End}(\mathcal{M})$};
   
   % Element of the vector space
   \path (M0) ++ (-0.8*\unit,0.5*\unit) node [dot] (x) {};
   \path (x.south)++(0,-0.1*\unit) node [below] {$\boldsymbol{\xi}$}; 
   
   % Element filtered in the vector space
   \path (M0) ++ (0.8*\unit,0.5*\unit) node [dot] (ex) {};
   \path (ex.south) node [below] {$\mathbf{D}_{\mathbf{F}\vert\mathbf{S}_i}\{\boldsymbol{\xi}\}$};      
              



   % Space of endomorphisms
   \path (M0.north) ++ (0, 0.5*\unit) 
         node [endomorphisms, anchor=south] (End0) {};
   \path (End0.north) ++ (0.0, 0) node [below] {$\text{End}\left(\text{End}(\mathcal{M})\right)$}; 
   

   % Adding an endomorphism element 
   \path (End0.south) ++ (0.0, 0.3*\unit) node [dot] (e) {};      
   \path (e) node [above] {$\mathbf{D}_{\mathbf{F}\vert\mathbf{S}_i}$};    
   
   % Arrow going from x to Ex
   \path (e)+(-0.5*\unit,0.45*\unit) coordinate (c1);
   \path (e)+(0.5*\unit,0.45*\unit) coordinate (c2);   
   \path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x) .. controls (c1) and (c2) .. (ex);   



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% SECOND COLUMN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Vector space 
\path (M0) ++ (\layerinterdist, 0) node [vectorspace] (M1) {};
\path (M1.south) ++ (0, 0) node [above] {$\bigoplus_{i=1}^{\text{dim}(\mathcal{M})}\mathcal{M}$};

% Element of the vector space
\path (M1) ++ (-0.8*\unit,0.5*\unit) node [dot] (x1) {};
\path (x1.south)++(0,-0.1) node [below] {$\vec{\boldsymbol{\xi}}$}; 

% Element filtered in the vector space
\path (M1) ++ (0.8*\unit,0.5*\unit) node [dot] (ex1) {};
\path (ex1.south) node [below] {$\overline{\mathbf{D}}_{\mathbf{F}\vert\mathbf{S}_i}\{\vec{\boldsymbol{\xi}}\}$};  



 % Space of endomorphisms
\path (End0) ++ (\layerinterdist, 0) 
node [endomorphisms] (End1) {};
\path (End1.north) ++ (0.0, 0) node [below] {$\text{End}\left( \bigoplus_{i=1}^{\text{dim}(\mathcal{M})}\right)$}; 

% Adding an endomorphism element 
\path (End1.south) ++ (0.0, 0.3*\unit) node [dot] (e1) {};      
\path (e1) node [above] {$\overline{\mathbf{D}}_{\mathbf{F}\vert\mathbf{S}_i}$};    

% Arrow going from x to Ex
\path (e1)+(-0.5*\unit,0.45*\unit) coordinate (c1);
\path (e1)+(0.5*\unit,0.45*\unit) coordinate (c2);   
\path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x1) .. controls (c1) and (c2) .. (ex1);   




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% THIRD COLUMN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 



% Vector space 
\path (M1) ++ (\layerinterdist, 0) node [vectorspace] (M2) {};
\path (M2.south) ++ (0, 0) node [above] {$\bigoplus_{i=1}^{\text{dim}(\mathcal{M})}\mathcal{M}$};

% Element of the vector space
\path (M2) ++ (-0.8*\unit,0.5*\unit) node [dot] (x2) {};
\path (x2.south)++(0,-0.1*\unit) node [below] {$\vec{\boldsymbol{\xi}}$}; 

% Element filtered in the vector space
\path (M2) ++ (0.8*\unit,0.5*\unit) node [dot] (ex2) {};
\path (ex2.south) node [below] {$\overline{\mathbf{D}}_{\mathbf{F}\vert\mathbf{S}_i}\{\vec{\boldsymbol{\xi}}\}$};  



% Space of endomorphisms
\path (End1) ++ (\layerinterdist, 0) 
node [endomorphisms] (End2) {};
\path (End2.north) ++ (0.0, 0) node [below] {$\text{End}(\mathcal{M})^{\ast}\otimes\text{End}(\mathcal{M})$}; 

% Adding an endomorphism element 
\path (End2.south) ++ (0.0, 0.3*\unit) node [dot] (e2) {};      
\path (e2) node [above] {$\overline{\mathbf{D}}_{\mathbf{F}\vert\mathbf{S}_i}$};    

% Arrow going from x to Ex
\path (e2)+(-0.5*\unit,0.45*\unit) coordinate (c1);
\path (e2)+(0.5*\unit,0.45*\unit) coordinate (c2);   
\path [draw, -stealth, line width=0.5,color=my_alejocol5a] (x2) .. controls (c1) and (c2) .. (ex2);   






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% ARROWS BETWEEN COLUMNS %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

 % Arrow going from a to e = \rho(a)
  
\path [draw, -stealth, line width = 1.0, green!50!black] 
(e) edge [bend right] node [below] {$I_1~~~$} (e1);


\path [draw, -stealth, line width = 1.0, green!50!black] 
(e1) edge [bend right] node [below] {$I_2~~~$} (e2);


\path [draw, -stealth, line width = 1.0, my_alejocol3a] 
(x) edge [bend right] node [below] {$\iota_1~~~$} (x1);

\path [draw, -stealth, line width = 1.0, my_alejocol3a] 
(x1) edge [bend right] node [below] {$\text{Id}~~~$} (x2);





\end{tikzpicture}

}



==> source_figs/plots_stability/frequency_response_change_graph_again.tex <==
%!TEX root = ../gnn_nyu_workshop_2019.tex

\def \thisplotscale {4}
\def \unit {\thisplotscale cm}

\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 0.8*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {-0.02, 0.45, 6.10, 6.9},
             xticklabels = {$\lam_0$, $\lam_1$, $\lam_k$, $\lam_{n-1}$},
             ymin = -0, ymax = 1.15,
             ytick = {-1}]
\addplot+[color = blue!50, ycomb, mark=*, mark options={blue!50}]
      coordinates { (-0.02, 0.9)
                    (0.45, 0.95)
                    (0.91+0.3*rand, 0.90)
                    (1.25+0.3*rand, 0.80)
                    (1.57+0.3*rand, 0.60)
                    (2.31+0.3*rand, 0.40)
                    (2.63+0.3*rand, 0.15)
                    (3.37+0.3*rand, 0.10)
                    (3.97+0.3*rand, 0.05)
                    (4.23+0.3*rand, 0.05)
                    (4.51+0.3*rand, 0.10)
                    (5.15+0.3*rand, 0.30)
                    (5.60+0.3*rand, 0.50)
                    (6.10, 1.00)
                    (6.72+0.3*rand, 0.9)
                    (6.9, 0.7)};

\addplot[domain=-0.5:7.5,samples = 80, color = red]
      { 0.8*exp(-(1*(x-1.2))^2) + 0.7*exp(-(0.7*(x-4))^2) + + 0.8 *exp(-(1.1*(x-6))^2)};

\end{axis}
\end{tikzpicture}






==> source_figs/plots_stability/frequency_response_instantiation.tex <==
%!TEX root = ../stability.tex

\def \thisplotscale {3.68}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8*exp(-(1*(x-1.2))^2) 
       + 0.7*exp(-(0.7*(x-4))^2) 
       + 0.8*exp(-(1.1*(x-6))^2) 
       + 0.1}


\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0, 0.45, 2.63, 3.37, 6.72, 7.20},
             xticklabels = {\blue{$\lam_1\phantom{\hlam}$}, 
                            \red{$\hlam_1$}, 
                            \blue{$\lam_i\phantom{\hlam}$}, 
                            \red{$\hlam_i$},
                            \blue{$\lam_{N}\phantom{\hlam}$},
                            \red{$\hlam_N$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             typeset ticklabels with strut,
             enlarge x limits=false]

\addplot+[samples at = {0.00, 0.91, 1.57, 
                        2.63, 3.97, 4.51, 
                        5.60, 6.72}, 
          color = blue!60, 
          ycomb, 
          mark=otimes*, 
          mark options={blue!60}]
         {\frequencyresponse};

\addplot+[samples at = {0.45, 1.25, 2.31, 
                        3.37, 4.23, 5.15, 
                        6.20, 7.20}, 
          color = red!60, 
          ycomb, 
          mark=oplus*, 
          mark options={red!60}]
         {\frequencyresponse};

\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> source_figs/plots_stability/graph_dilation_one.tex <==
%!TEX root = ../gnn_nyu_workshop_2019.tex

\def \thisplotscale {4}
\def \unit {\thisplotscale cm}

\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 0.8*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0, 0.45, 6.20, 7.20},
             xticklabels = {$\lam_0$, $\lam_1$, $\lam_k$, $\lam_{n-1}$},
             ymin = -0, ymax = 1.15,
             ytick = {-1}]
\addplot+[color = blue!50, ycomb, mark=*, mark options={blue!50}]
      coordinates { (0.00, 0.9)
                    (0.45, 0.95)
                    (0.91, 0.90)
                    (1.25, 0.80)
                    (1.57, 0.60)
                    (2.31, 0.40)
                    (2.63, 0.15)
                    (3.37, 0.10)
                    (3.97, 0.05)
                    (4.23, 0.05)
                    (4.51, 0.10)
                    (5.15, 0.30)
                    (5.60, 0.50)
                    (6.20, 1.00)
                    (6.72, 0.9)
                    (7.20, 0.7)};

\addplot[domain=-0.5:7.5,samples = 80, color = red]
      { 0.8*exp(-(1*(x-1.2))^2) + 0.7*exp(-(0.7*(x-4))^2) + + 0.8 *exp(-(1.1*(x-6))^2)};

\end{axis}
\end{tikzpicture}





==> source_figs/plots_stability/graph_dilation_unstable.tex <==
%!TEX root = ../stability.tex

%Defining my own colors
\colorlet{my_blue}{blue!50!cyan}
\definecolor{my_red}{rgb}{1, 0, 0.4980}

\def \thisplotscale {3.6}
\def \unit {\thisplotscale cm}

\def \frequencyresponse 
     {   0.8*exp(-(1*(x-1.2))^2) 
      -0.2*exp(-(0.5*(x-7))^2)+0.5*exp(-(1*(x))^2)
       + 0.7*exp(-(0.7*(x-4))^2) 
       + 0.8*exp(-(1.4*(x-6))^2) 
       + 0.1}

\hspace{-2.9mm}
\begin{tikzpicture}[x = 1*\unit, y=1*\unit]

\def \factorx {2.4/8}
\def \deltax  {0.5*\factorx}
\def \shadeshift  {0.05}

\path [fill=black!20, opacity = 0.5] 
              (\deltax - 0.001*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 0.030*\factorx + \shadeshift, 1.00);
\path [fill=black!20, opacity = 0.5] 
              (\deltax + 3.393*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 3.770*\factorx + \shadeshift, 1.00);
\path [fill=black!20, opacity = 0.5] 
              (\deltax + 6.048*\factorx - \shadeshift, 0.00) rectangle 
              (\deltax + 6.720*\factorx + \shadeshift, 1.00);

\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 1*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0.03, -0.01, 3.77, 3.393, 6.72, 6.048},
             xticklabels = {\red{$\quad\quad\vert\tilde{\lam}_1\vert\phantom{\lam}$},
                            \blue{$\vert\lam_1\vert\quad\quad$}, 
                            \red{$\quad\tilde{\lam}_i\vert\phantom{\lam}$}, 
                            \blue{$\vert\lam_i\vert$},
                            \red{$\quad\vert\tilde{\lam}_{N}\vert\phantom{\lam}$},
                            \blue{$\vert\lam_N\vert$}},
             ymin = -0, ymax = 1.15,
             ytick = {-1},
             typeset ticklabels with strut,
             enlarge x limits=false]

\addplot+[samples at = {0.03, 0.91, 1.57, 
                        2.63, 3.77, 4.51, 
                        5.60, 6.72}, 
          color = my_red, 
          ycomb, 
          mark=otimes*, 
          mark options={my_red}]
         {\frequencyresponse};

\addplot+[samples at = {-0.01, 0.819, 1.413, 
                        2.367, 3.393, 4.059, 
                        5.04, 6.048}, 
          color = my_blue, 
          ycomb, 
          mark=oplus*, 
          mark options={my_blue}]
         {\frequencyresponse};

\addplot[ domain=-0.5:7.5, 
          samples = 80, 
          color = black,
          line width = 1.2]
         {\frequencyresponse};


\end{axis}
\end{tikzpicture}


%{-0.22, 0.25, 0.61, 1.05, 1.37, 2.11, 
%  2.43, 3.07, 3.67, 4.13, 4.31, 5.05, 
%  5.20, 6.00, 6.42, 7.00}



==> source_figs/plots_stability/large_frequency_features.tex <==
%!TEX root = ../gnn_nyu_workshop_2019.tex

\def \thisplotscale {4}
\def \unit {\thisplotscale cm}

\begin{tikzpicture}[x = 1*\unit, y=1*\unit]
\begin{axis}[scale only axis,
             width  = 2.4*\unit,
             height = 0.8*\unit,
             xmin = -0.5, xmax=7.5,
             xtick = {0, 0.45, 6.20, 7.20},
             xticklabels = {$\lam_0$, $\lam_1$, $\lam_k$, $\lam_{n-1}$},
             ymin = -0, ymax = 1.15,
             ytick = {-1}]
\addplot+[color = blue!30, ycomb, mark=*, mark options={blue!30}]
      coordinates { (0.00, 0.0)
                    (0.45, 0.0)
                    (0.91, 0.0)
                    (1.25, 0.0)
                    (1.57, 0.0)
                    (2.31, 0.0)
                    (2.63, 0.0)
                    (3.37, 0.0)
                    (3.97, 0.0)
                    (4.23, 0.0)
                    (4.51, 0.0)
                    (5.15, 0.0)
                    (5.60, 0.0)
                    (6.20, 1.00)
                    (6.72, 0.0)
                    (7.20, 0.0)};

\addplot+[color = blue!60, ycomb, mark=*, mark options={blue!60}]
      coordinates { (6.20, 1*1.00) };


\addplot+[color = mygreen!60, ycomb, mark=*, mark options={mygreen!60}]
      coordinates {(0.9*6.20, 1*1.00)};


\addplot[domain=5:8,samples = 80, color = red]
      { 1.1*exp(-(2.5*(x-6.2))^2)};

\end{axis}
\end{tikzpicture}
















==> v25/sec_Spectral_Representation_Filtersc.tex <==
%!TEX root = ../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Spectral Representations of Filters}

==> v25/sec_conclusions.tex <==
%!TEX root = ../compiler_paper.tex





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% CONCLUSIONS %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Conclusions}\label{sec:conclusions}

We obtained stability bounds for algebraic neural networks (AlgNN) considering unital associative algebras that are not necessarily commutative. These findings extend the results found in~\cite{parada_algnn} which were obtained for commutative algebras. Additionally, the bounds presented in this paper are tighter than those obtained in~\cite{parada_algnn}. Additionally we show that the non commutativity between shift operators and between the shift operators and the perturbation $\bbT(\bbS)$ does not affect the stability bounds. This also has a strong implication for the stability bounds derived in~\cite{fern2019stability} for graph neural networks (GNNs).








